Improving Context-Based Meta-Reinforcement Learning with Self-Supervised Trajectory Contrastive Learning

Meta-reinforcement learning typically requires orders of magnitude more samples than single task reinforcement learning methods. This is because meta-training needs to deal with more diverse distributions and train extra components such as context encoders. To address this, we propose a novel self-supervised learning task, which we named Trajectory Contrastive Learning (TCL), to improve meta-training. TCL adopts contrastive learning and trains a context encoder to predict whether two transition windows are sampled from the same trajectory. TCL leverages the natural hierarchical structure of context-based meta-RL and makes minimal assumptions, allowing it to be generally applicable to context-based meta-RL algorithms. It accelerates the training of context encoders and improves meta-training overall. Experiments show that TCL performs better or comparably than a strong meta-RL baseline in most of the environments on both meta-RL MuJoCo (5 of 6) and Meta-World benchmarks (44 out of 50).

==> tables/metaworld_wins.tex <==
\begin{tabular}{l|ccccc}
\toprule
{} &              MAML &             RL2 &              MQL &            PEARL &        TCL-PEARL \\
\midrule
Wins             &   4 &               6 &                4 &                4 &       \textbf{7} \\
\bottomrule
\end{tabular}
